Homology-Preserving Multi-Scale Graph Skeletonization Using Mapper on Graphs

Node-link diagrams are a popular method for representing graphs that capture relationships between individuals, businesses, proteins, and telecommunication endpoints. However, node-link diagrams may fail to convey insights regarding graph structures, even for moderately sized data of a few hundred nodes, due to visual clutter. We propose to apply the mapper construction -- a popular tool in topological data analysis -- to graph visualization, which provides a strong theoretical basis for summarizing the data while preserving their core structures. We develop a variation of the mapper construction targeting weighted, undirected graphs, called {\mog}, which generates homology-preserving skeletons of graphs. We further show how the adjustment of a single parameter enables multi-scale skeletonization of the input graph. We provide a software tool that enables interactive explorations of such skeletons and demonstrate the effectiveness of our method for synthetic and real-world data.

==> fig.small_graphs.tex <==



\begin{figure*}[!t]
    \centering

\subfloat[\textsc{barbell graph(50,20)}: Fiedler vector, connected components]{
    \begin{minipage}[t]{0.118\linewidth} \centering
        \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_barbell_graph(50,20)_mog_fv_6.png}} {\tiny $\epsilon\!=\!0, n\!=\!6$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering
        \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_barbell_graph(50,20)_mog_fv_10.png}} {\tiny $\epsilon\!=\!0, n\!=\!10$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering
        \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_barbell_graph(50,20)_mog_fv_20.png}} {\tiny $\epsilon\!=\!0, n\!=\!20$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering
        \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_barbell_graph(50,20)_graph_fv.png}} {\tiny Input Graph}
    \end{minipage}
        
    }
    \hfill
    \subfloat[\textsc{bio-celegans}: PageRank, modularity clustering]{
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bio-celegans_mog_pr_0_85_2.png}}  {\tiny $\epsilon\!=\!0, n\!=\!2$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bio-celegans_mog_pr_0_85_20.png}} {\tiny $\epsilon\!=\!0, n\!=\!20$}
    \end{minipage}
\begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bio-celegans_mog_pr_0_85_40.png}} {\tiny $\epsilon\!=\!0, n\!=\!40$}
    \end{minipage}        
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bio-celegans_graph_pr_0_85.png}} {\tiny Input Graph}
    \end{minipage}
        
    } 
                

    \subfloat[\textsc{bio-diseasome}: Fiedler vector, modularity clustering]{
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bio-diseasome_mog_fv_2.png}}  {\tiny $\epsilon\!=\!0, n\!=\!2$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bio-diseasome_mog_fv_8.png}}  {\tiny $\epsilon\!=\!0, n\!=\!8$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bio-diseasome_mog_fv_40.png}} {\tiny $\epsilon\!=\!0, n\!=\!40$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bio-diseasome_graph_fv.png}} {\tiny Input Graph}
    \end{minipage}
        
    }
    \hfill
    \subfloat[\textsc{hic 5k net 7}: density (equalized), connected components]{
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_hic_5k_net_7_mog_den_0_5_10.png}}  {\tiny $\epsilon\!=\!0, n\!=\!10$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_hic_5k_net_7_mog_den_0_5_20.png}}  {\tiny $\epsilon\!=\!0, n\!=\!20$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_hic_5k_net_7_mog_den_0_5_40.png}} {\tiny $\epsilon\!=\!0, n\!=\!40$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_hic_5k_net_7_graph_den_0_5.png}} {\tiny Input Graph}
    \end{minipage}

    }


    \subfloat[\textsc{collaboration network}: eccentricity, connected components]{
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_collaboration_network_mog_ecc_4.png}}  {\tiny $\epsilon\!=\!0, n\!=\!4$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering    
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_collaboration_network_mog_ecc_10.png}} {\tiny $\epsilon\!=\!0, n\!=\!10$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_collaboration_network_mog_ecc_40.png}} {\tiny $\epsilon\!=\!0, n\!=\!40$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_collaboration_network_graph_ecc.png}} {\tiny Input Graph}
    \end{minipage}

    }
    \hfill
    \subfloat[\textsc{bn-mouse-visual-cortex-2}: Fiedler vec.~(equalized), async.\ label prop.]{
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bn-mouse-visual-cortex-2_mog_fv_6.png}} {\tiny $\epsilon\!=\!0, n\!=\!6$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bn-mouse-visual-cortex-2_mog_fv_10.png}} {\tiny $\epsilon\!=\!0, n\!=\!10$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bn-mouse-visual-cortex-2_mog_fv_20.png}} {\tiny $\epsilon\!=\!0, n\!=\!20$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_bn-mouse-visual-cortex-2_graph_fv.png}} {\tiny Input Graph}
    \end{minipage}
        
        
    }
    
    
    \subfloat[\textsc{enron-email}: AGD, asynchronous label propagation]{
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_enron-email_mog_agd_8.png}} {\tiny $\epsilon\!=\!0, n\!=\!8$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_enron-email_mog_agd_10.png}} {\tiny $\epsilon\!=\!0, n\!=\!10$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_enron-email_mog_agd_20.png}} {\tiny $\epsilon\!=\!0, n\!=\!20$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_enron-email_graph_agd.png}} {\tiny Input Graph}
    \end{minipage}
        
        
    }
    \hfill
    \subfloat[\textsc{usair97}: AGD (equalized), modularity clustering]{
    \begin{minipage}[t]{0.118\linewidth} \centering    
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_usair97_mog_agd_3.png}}  {\tiny $\epsilon\!=\!0, n\!=\!2$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering        
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_usair97_mog_agd_8.png}}  {\tiny $\epsilon\!=\!0, n\!=\!8$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_usair97_mog_agd_20.png}} {\tiny $\epsilon\!=\!0, n\!=\!20$} 
    \end{minipage} \hfill
    \begin{minipage}[t]{0.118\linewidth} \centering
        \fbox{\includegraphics[width=0.95\linewidth]{figs/fig11/fig11_usair97_graph_agd.png}} {\tiny Input Graph}
    \end{minipage}

        
    }
    
    \caption{A series of small input graphs demonstrating how \mog retains prominent topological structure of the input graph as the number of cover elements, $n$, is varied.}
    \label{fig:small_graphs}
\end{figure*}



